DeepDive: An Integrative Algorithm/Architecture Co-Design for Deep Separable Convolutional Neural Networks

Deep Separable Convolutional Neural Networks (DSCNNs) have become the emerging paradigm by offering modular networks with structural sparsity in order to achieve higher accuracy with relatively lower operations and parameters. However, there is a lack of customized architectures that can provide flexible solutions that fit the sparsity of the DSCNNs. This paper introduces DeepDive, which is a fully-functional, vertical co-design framework, for power-efficient implementation of DSCNNs on edge FPGAs. DeepDive's architecture supports crucial heterogeneous Compute Units (CUs) to fully support DSCNNs with various convolutional operators interconnected with structural sparsity. It offers an FPGA-aware training and online quantization combined with modular synthesizable C++ CUs, customized for DSCNNs. The execution results on Xilinx's ZCU102 FPGA board, demonstrate 47.4 and 233.3 FPS/Watt for MobileNet-V2 and a compact version of EfficientNet, respectively, as two state-of-the-art depthwise separable CNNs. These comparisons showcase how DeepDive improves FPS/Watt by 2.2$\times$ and 1.51$\times$ over Jetson Nano high and low power modes, respectively. It also enhances FPS/Watt about 2.27$\times$ and 37.25$\times$ over two other FPGA implementations. The DeepDive output for MobileNetV2 is available at https://github.com/TeCSAR-UNCC/DeepDive.

==> tex/ExpRes/Tables/effNet_mapping.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Mapping \effnet~to Hardware Accelerators.  PS is Processing System and PL is Programmable logic}
%     \begin{adjustbox}{width=1.0\linewidth,center}
%     \begin{tabular}{clcc}
%     \toprule
%     \toprule
%     Item & \multicolumn{1}{c}{Compute Units} & Compressed \effnet~& Implementation \\
%     \midrule
%     1 & Head CU & 1 & PL \\
%     2 & Body CU & 1 & PL \\
%     3 & Tail CU & 9 & PL \\
%     4 & Classifier & 1 & PS \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:effnet_mapping}%
%   \end{adjustbox}
% \end{table}%



==> tex/ExpRes/Tables/vta_deepDive.tex <==
% Table generated by Excel2LaTeX from sheet 'PaperTable'
\begin{table}[htbp]
  \centering
  \caption{Energy efficiency comparison of VTA running ResNet-18 with input size of 224 and DeepDive running design point ($H=224, \alpha=0.75$)}
  \begin{adjustbox}{width=\linewidth,center}
    \begin{tabular}{cccc|cccc}
    \toprule
    \toprule
    \multicolumn{4}{c}{VTA(ResNet-18, 224)} & \multicolumn{4}{c}{DeepDive($H=224, \alpha=0.75$)} \\
    \midrule
    Top1(\%) & Power(W) & FPS & FPS/W & Top1(\%) & Power(W) & FPS & FPS/W\\
    69.92 & 1.47  & 15.44 & 10.51 & 66.4  & 0.46  & 11    & 23.91 \\
    \bottomrule
    \end{tabular}%
  \label{tab:vta}%
  \end{adjustbox}
\end{table}%


==> tex/ack.tex <==
 \section*{Acknowledgments}
The authors would like to thank...


==> tex/biography.tex <==


\vspace{-2cm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./Figs/Bio/baharani}}]{Mohammadreza Baharani}
(S’18)
received the M.Sc. degree in computer engineering
from University of Tehran, Iran, in 2012. He is currently a Ph.D. student in the TeCSAR group at the Department of Electrical and Computer Engineering, University of North Carolina at Charlotte, USA. He carries out researches on embedded system design, Applied AI, VLSI realization of machine learning algorithms for embedded purposes, performance, power and thermal management of multi-core processors.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{./Figs/Bio/tabkhi_hamed}}]{Hamed Tabkhi}
(S’07–M’14)
is an Assistant Professor in the Department of Electrical and Computer Engineering, University of North Carolina at Charlotte, USA.
He was a post-doctoral research associate at Northeastern University. Hamed Tabkhi received his Ph.D. degree in 2014 from Northeastern University under the direction of Prof. Gunar Schirner. Overall, his research focuses on transformative computer systems and architecture for cyber-physical, real-time streaming and emerging machine learning applications.
\end{IEEEbiography}



%%%%%%%%%%% draft.bib %%%%%%%%%%%%%%%%%%%



% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks




